EMaQ: Expected-Max Q-Learning Operator for Simple Yet Effective Offline and Online RL

Off-policy reinforcement learning holds the promise of sample-efficient learning of decision-making policies by leveraging past experience. However, in the offline RL setting -- where a fixed collection of interactions are provided and no further interactions are allowed -- it has been shown that standard off-policy RL methods can significantly underperform. Recently proposed methods often aim to address this shortcoming by constraining learned policies to remain close to the given dataset of interactions. In this work, we closely investigate an important simplification of BCQ -- a prior approach for offline RL -- which removes a heuristic design choice and naturally restricts extracted policies to remain exactly within the support of a given behavior policy. Importantly, in contrast to their original theoretical considerations, we derive this simplified algorithm through the introduction of a novel backup operator, Expected-Max Q-Learning (EMaQ), which is more closely related to the resulting practical algorithm. Specifically, in addition to the distribution support, EMaQ explicitly considers the number of samples and the proposal distribution, allowing us to derive new sub-optimality bounds which can serve as a novel measure of complexity for offline RL problems. In the offline RL setting -- the main focus of this work -- EMaQ matches and outperforms prior state-of-the-art in the D4RL benchmarks. In the online RL setting, we demonstrate that EMaQ is competitive with Soft Actor Critic. The key contributions of our empirical findings are demonstrating the importance of careful generative model design for estimating behavior policies, and an intuitive notion of complexity for offline RL problems. With its simple interpretation and fewer moving parts, such as no explicit function approximator representing the policy, EMaQ serves as a strong yet easy to implement baseline for future work.

==> algs/y_target.tex <==
% \begin{algorithm}[t]
%   \DontPrintSemicolon
%   \SetKwProg{Fn}{Function}{:}{}
  
%   \SetKwFunction{fEnsemble}{Ensemble}
%     \Fn{\fEnsemble{values}}{
%         \KwRet $\lambda \cdot \min(values) + (1-\lambda) \cdot \max(values)$\;
%     }

%   \SetKwFunction{FMain}{$y_{\textnormal{target}}$}
%   \Fn{\FMain{$s,a,s',r,t$}}{
%         $\{a'_i\}^N \sim \mu(a'|s')$\;
%         $Qvalues \gets [\quad]$\;
%         \For{$k\gets1$ \KwTo $N$}{
%             \tcc{Estimate the value of action $a'_k$}
%             $Qvalues.\texttt{append}\Big(\fEnsemble\big([Q^{target}_i(s', a'_k) \textnormal{ for all } i]\big)\Big)$\;
%         }
%         \KwRet $r + (1-t) \cdot \gamma \max(Qvalues)$\;
%   }
%   \;
%   \caption{Computing EMaQ $y_{\textnormal{target}}$
%   %\vspace{-0.5cm}
%   }
%   \label{alg:ytarget}
% \end{algorithm}

\begin{algorithm}[t]
  \DontPrintSemicolon
  
  Offline dataset $\mathcal{D}$, Pretrain $\muas$ on $\mathcal{D}$\;
  Initialize $K$ Q functions with parameters $\theta_i$, and $K$ target Q functions with parameters $\theta^{\textnormal{target}}_i$\;
  $\texttt{Ensemble}$ parameter $\lambda$, Exponential moving average parameter $\alpha$\;\;
  
  \SetKwProg{Fn}{Function}{:}{}
  
  \SetKwFunction{fEnsemble}{Ensemble}
    \Fn{\fEnsemble{values}}{
        \KwRet $\lambda \cdot \min(values) + (1-\lambda) \cdot \max(values)$\;
    }

  \SetKwFunction{FMain}{$y_{\textnormal{target}}$}
  \Fn{\FMain{$s,a,s',r,t$}}{
        $\{a'_i\}^N \sim \mu(a'|s')$\;
        $Qvalues \gets [\quad]$\;
        \For{$k\gets1$ \KwTo $N$}{
            \tcc{Estimate the value of action $a'_k$}
            $Qvalues.\texttt{append}\Big(\fEnsemble\big([Q^{target}_i(s', a'_k) \textnormal{ for all } i]\big)\Big)$\;
        }
        \KwRet $r + (1-t) \cdot \gamma \max(Qvalues)$\;
  }
  \;
  \While{not converged}{
    Sample a batch $\{(s_m,a_m,s'_m,r_m,t_m)\}^M \sim \mathcal{D}$\;
    \For{$i=1,...,K$}{
        $\mathcal{L}(\theta_i) = \sum_m \Big(Q_i(s_m,a_m) - y_{\textnormal{target}}(s_m,a_m,s'_m,r_m,t_m)\Big)^2$\;
        $\theta_i \leftarrow \theta_i - \texttt{AdamUpdate}\Big(\mathcal{L}(\theta_i), \theta_i\Big)$\;
        $\theta^{\textnormal{target}}_i \leftarrow \alpha \cdot \theta^{\textnormal{target}}_i + (1 - \alpha) \cdot \theta_i$\;
    }
  }
  \caption{
    Full EMaQ Training Algorithm
  }
  \label{alg:ytarget}
\end{algorithm}


==> background.tex <==
\section{Old Background}
    Throughout this work, we represent Markov Decision Process (MDP) as $M = \langle \mathcal{S}, \mathcal{A}, r, \mathcal{P}, \gamma \rangle$, with state space $\mathcal{S}$, action space $\mathcal{A}$, reward function $r: \mathcal{S} \!\times\!\mathcal{A}\! \rightarrow\! \mathds{R}$, transition dynamics $\mathcal{P}$, and discount %factor
    $\gamma$.
    
    \paragraph{Q-Evaluation and Q-Learning}
        The standard Q-Evaluation and Q-Learning backup operators in RL have the following forms:
        \begin{align*}
            \mbox{Q-Evaluation for policy $\mu$}\qquad &\mathcal{T}_\mu Q(s,a) := r(s,a) + \gamma \cdot \mathds{E}_{s'}\mathds{E}_{a' \sim \mu} \Big[Q(s',a')\Big]\\
            \mbox{Q-Learning}\qquad  &\mathcal{T}^*Q(s,a) := r(s,a) + \gamma \cdot \mathds{E}_{s'}\Big[\max_{a'} Q(s',a')\Big]
        \end{align*}
        As will be seen below, by devising an interpolation between $\mathds{E}_{s'}\mathds{E}_{a' \sim \mu} [Q(s',a')]$ and $\mathds{E}_{s'}[\max_{a'} Q(s',a')]$, our proposed operator EMaQ becomes an interpolant of these operators.
    
    \paragraph{Batch Constrained Q-Learning (BCQ)\citep{fujimoto2018off}} BCQ is a successful method for fully off-policy RL. To constrain learned policies to remain close to the offline dataset, policies are parameterized as:
    \begin{align*}
        \pi_\theta(a|s) = \argmax_{a_i + \xi_\theta(s,a_i)} Q_\psi(s,a_i + \xi_\theta(s,a_i)) \qquad \mbox{for} \qquad a_i \sim \mu(a|s), i=1, ..., N
    \end{align*}
    where $Q_\psi$ is a learned, $\muas$ is a base behavior policy (a generative model trained on the dataset), and $\xi_\theta$ is an MLP that learns to perturb sampled actions towards more optimal actions. Most importantly, the output of $\xi_\theta$ is bounded with a range $[-\Phi,\Phi]$, controlling how far the policy can deviate from $\muas$. $\muas$ is learned with the generative modelling objective, and the remaining models are learned through RL updates resembling the TD3 algorithm \citep{fujimoto2018addressing}.
    
    \paragraph{Bootstrapping Error Accumulation Reduction (BEAR)\citep{kumar2019stabilizing}} Constraining policies in the manner of BCQ %may become too
    is quite
    restrictive and choosing an appropriate value of $\Phi$ %may be 
    proves
    challenging
    in practice. 
    In BEAR, the driving intuition is that rather than constraining learned policies $\pi$ to be close to the behavior policy $\muas$, it would be more effective to constrain the support of learned policies to match the support of $\muas$; the policy could then deviate significantly from $\muas$ while being constrained to the support of the data distribution. Practically, this is implemented by %upper
    bounding the deviation in terms of Maximum Mean Discrepancy \citep{gretton2012kernel}. The proposed policy takes the %following
    form:
    \begin{align*}
        \max_\pi \mathds{E}_{s \sim \mathcal{D}}\mathds{E}_{\pi(a|s)} \Big[\min_{j=1,...,K}Q_j(s,a)\Big] \qquad \mbox{s.t.} \qquad \mathds{E}_{s \sim \mathcal{D}}\Big[\textnormal{MMD}(\mu(\cdot|s), \pi(\cdot|s))\Big] \leq \epsilon
    \end{align*}
    where $\mathcal{D}$ denotes the offline dataset and $Q_j$ are learned through RL updates resembling the TD3 algorithm~\citep{fujimoto2018addressing}. The policy objective is optimized through dual gradient descent. It can be challenging to balance the needed value of $\epsilon$ with respect to the scale of rewards in the MDP, and similar to the $\Phi$ variable in BCQ, the choice may need to be state-dependent. Lastly, matching the support of $\muas$ may %in some case 
    be 
    overly
    restrictive and we may need to allow policies to only cover a subset of the support.
    
    %\paragraph{Behavior Regularized Actor Critic (BRAC)\citep{wu2019behavior}} {\color{blue} WE ARE RUNNING OUT OF SPACE AND IDK IF WE NEED TO TALK ABOUT THIS?}


==> broader_impact.tex <==
\section*{Broader Impact}

Offline RL is an important area of research in reinforcement learning, as its problem setting is more suited for learning from costly real-world data, 
 such as in robotics~\cite{gu2017deep,kalashnikov2018qtopt}, health~\cite{murphy2001marginal}, dialog agents~\citep{jaques2019way}, and education~\cite{mandel2014offline}.
We provide a novel algorithm that achieves competitive state-of-the-art performances while remaining simple enough for theoretical analyses.
As offline RL with rich function approximators is a fledgling field~\citep{fujimoto2018off,levine2020offline}, it poses many unanswered questions and we hope our work can serve as a simple starting point for both
empirical and theoretical investigations. Other impact questions are not applicable for this paper.

% {\color{blue}{\textbf{THIS IS A MANDATORY THING AND HAS TO BE FILLED OUT}}}

% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}


==> intriguing_findings.tex <==
% \vspace{-0.3cm}
\subsection{\texorpdfstring{$\bigstar\bigstar$}{**} Intriguing Results Observed Through EMaQ \texorpdfstring{$\bigstar\bigstar$}{**}}
    \paragraph{Gauging Difficulty of Offline RL Tasks} A very eye-catching result in above figures is that \textbf{in almost all settings of the standard Mujoco environments (Figures \ref{fig:ablation} and \ref{fig:mujocoplots}), $\bm{N=5}$ significantly improves upon $\bm{\muas}$ and in most settings matches or exceeds significantly beyond previously reported results}. In the medium-expert setting this may have been expected: After the initial timesteps, the trajectories for medium and expert behavior policies may deviate in the state-space, making $\muas$ behave as the expert in those states; if the learned policy could make the right decisions in the first timesteps, it could then remain close to $\muas$ and be a very good policy. However, the results in the random, medium, and mixed settings suggest that \textbf{EMaQ with very low values of $\bm{N}$ may be useful as a litmus test for understanding to what extent the base behavior policy needs to be modified for obtaining a performant policy}.
    
    \paragraph{Choice of Generative Model} The practical rendition of EMaQ consists of only two components: a pretrained base behavior policy $\muas$, and MLP Q functions. As such, the generative model used to represent $\muas$ becomes an even more central component compared to prior approaches which train an additional actor (or residual actor)~\citep{fujimoto2018off,wu2019behavior,kumar2019stabilizing}. In experiments presented in Appendix \ref{ap:vae_results}, we replaced our choice of autoregressive generative model architecture with a VAE of similar parameter-count. While the two types of $\muas$ obtain similar performance when evaluated in the environments, EMaQ does not succeed in improving upon $\muas$ when it is represented as a VAE.
    We do not believe that autoregressive models are intrinsically better than VAEs, but rather our results demonstrate the need for more careful attention on the choice of $\muas$.
    \textbf{Since EMaQ is closely tied to the choice of behavior model, it may be valuable for evaluating how well $\bm{\muas}$ represents the given offline dataset.}
    \textbf{From a practical perspective, our results suggest that for a given domain, focusing efforts on building-in good inductive biases in the generative models and value functions might be sufficient to obtain strong offline RL performance in many domains.}
    
    % \paragraph{Need for Better Out of Distribution Detection} Figure \ref{fig:mu_seed_problem} demonstrates that when using larger values of $N$ in EMaQ, we observe a distinct difference in performance across generative models trained with different random seeds. Since the only models involed in EMaQ are the generative model $\mu$ and learned Q-functions, we attribute this problem to the ensembling approach used to combat over-estimation of Q-values. Our ensembling approach is borrowed from recent literature \citep{fujimoto2018addressing, fujimoto2018off, kumar2019stabilizing}
    
    % \begin{figure}[t]
    %     \centering
    %     \includegraphics[width=\textwidth]{figs/mu_seed_problem.png}
    %     \caption{\small
    %         This problem while also observed in the kitchen-mixed setting, is particularly pronounced in the kitchen-partial setting.
    %     }
    %     \label{fig:mu_seed_problem}
    % \end{figure}
    
    
    
    
    
    % many scenarios is close to what the best $\bm{N}$ achieves

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

